Aspect-based Academic Search using Domain-specific KB

Academic search engines allow scientists to explore related work relevant to a given query. Often, the user is also aware of the "aspect" to retrieve a relevant document. In such cases, existing search engines can be used by expanding the query with terms describing that aspect. However, this approach does not guarantee good results since plain keyword matches do not always imply relevance. To address this issue, we define and solve a novel academic search task, called "aspect-based retrieval", which allows the user to specify the aspect along with the query to retrieve a ranked list of relevant documents. The primary idea is to estimate a language model for the aspect as well as the query using a domain-specific knowledge base and use a mixture of the two to determine the relevance of the article. Our evaluation of the results over the Open Research Corpus dataset shows that our method outperforms keyword-based expansion of query with aspect with and without relevance feedback.

==> Aspect-based Academic Search using Domain-specific KB/conclusion.tex <==
%\vspace*{-4mm}
\section{Conclusion}
\label{sec:con}
%\vspace{-2mm}
In this paper, we built an aspect-based retrieval model for scientific literature using TeKnowbase. Given a query and an aspect, this model returns a ranked list of documents that address that aspect for the query. We tested our model for 43 queries and 3 aspects with satisfactory results. We could beat the results obtained by adding aspect name explicitly to the query and doing pseudo-relevance feedback on those documents. 

\noindent\textbf{Acknowledgements}\\
This work was partially supported by IIT Delhi-IBM Research AI Horizons Network collaborative grant;  Ramanujan Fellowship, DST (ECR/2017/00l691) and the Infosys Centre for AI, IIIT-Delhi, India. T. Chakraborty would like to thank the support of Google India Faculty Award. 



==> Aspect-based Academic Search using Domain-specific KB/experiments.tex <==
%\vspace*{-6mm}
\section{Experiments}
\label{sec:experiment}
%\vspace*{-4mm}
\subsection{Setup}
{\bf Dataset.}
We used the Open Research Corpus dataset and indexed it using Galago. The baseline models (described below) are already implemented in Galago.\\
{\bf Aspects.}
We experimented with 3 different aspects -- \aspect{ application}, \aspect{algorithm} and \aspect{implementation}. We set $\lambda$ and $\beta$ to 0.5 in Eqs. \eqref{eq:model_eq} and \eqref{eq:mix_ent_prob}. We restricted ourselves to meta-paths of size at most 3.  We set $k$=5 for choosing the top-k meta-paths for generating embeddings using MetaPath2Vec (described in Section \ref{sec:metapath2vec}).\\
{\bf Benchmarks.}
Benchmark queries were taken from a set of 100 queries released by \cite{Xiong:2017:ESR:3038912.3052558} out of which 43 existed as whole entities in $TKB$, shown in Figure \ref{tab:benchmark}.
\small
\begin{figure*}[]
\vspace*{-5mm}
\centering
\begin{boxedminipage}[c]{\textwidth}
\term{artificial intelligence}, \term{augmented reality},  \term{autoencoder}, \term{big data}, \term{category theory}, 
\term{clojure}, \term{cnn}, \term{computer vision}, \term{cryptography}, \term{data mining},    
\term{data science}, \term{deep learning}, \term{differential evolution}, \term{dirichlet process}, \term{duality},
\term{genetic algorithm}, \term{graph drawing}, \term{graph theory}, \term{hashing}, \term{information geometry},
\term{information retrieval}, \term{information theory}, \term{knowledge graph}, \term{machine learning}, \term{memory hierarchy},
\term{mobile payment}, \term{natural language}, \term{neural network}, \term{ontology}, \term{personality trait},
\term{prolog}, \term{question answering}, \term{recommender system}, \term{reinforcement learning}, \term{sap},
\term{semantic web}, \term{sentiment analysis}, \term{smart thermostat}, \term{social media}, \term{speech recognition},
\term{supervised learning}, \term{variable neighborhood search}, \term{word embedding}
\end{boxedminipage}
\caption{Benchmark queries}
\label{tab:benchmark}
\vspace{-5mm}
\end{figure*}
\vspace{-2mm}
\normalsize

\noindent\textbf{Baselines.}
\label{sec:baseline}
We explicitly added the keyword representing the aspect to the query and used standard retrieval models with/without relevance feedback techniques as baselines described below:\\
{\bf 1) Query likelihood model with query only (QL+query).} Query likelihood \cite{Ponte:1998:LMA:290941.291008} estimates a language model for each document in the collection and ranks them by the likelihood of seeing the query terms as a random sample given that document model. 
\begin{comment}
Following is a brief overview of query-likelihood model. Using Bayes rule, we can write he likelihood of a document given a query as follows:

\begin{equation*}
    P(d|q) = \frac{P(q|d)P(d)}{P(q)}
\end{equation*}
Since $P(q)$ is the same for all the documents, we can ignore this term. $P(d)$ can be assumed to be uniform for all the documents. So, this can be ignored also. The final likelihood is given by Equation \eqref{eq:query_likelihood}. It is dirichlet smoothed with parameter $\mu$.

\begin{equation*}
    P(d|q) = P(q|d)
\end{equation*}

$P(q|d)$ is estimated as follows:

%\vspace*{-2mm}
\small
\begin{equation}
\label{eq:query_likelihood}
    P(d|q) \propto P(q|d) = \prod_{w \in terms(q)}\frac{tf(w)+\mu P(w|C)}{|d|+\mu}
\end{equation}
\normalsize
\end{comment}
\\
 {\bf 2) Query likelihood model with query + aspect name (QL + query + aspect).} We used the same model as above but added the terms \term{application}, \term{algorithm} or \term{implementation} to the query based on the aspect and retrieved the results. \\
 {\bf 3) Query expansion with pseudo relevance feedback on  QL + query + aspect (QL + query + aspect + QE).} We chose top-100 terms to expand the query for the query used in the previous baseline using relevance feedback model \cite{Lavrenko:2001:RBL:383952.383972}. Top-1000 documents were used as feedback documents. The weight of the original query was set as 0.75.
 
\noindent{\bf 4) Mixture Model (MM)}. This is our retrieval model described in Section \ref{sec:model}.
 \begin{comment}
 %\vspace{-5mm}
 \small
\begin{equation*}
    P(w|q_1,q_2,...,q_k) = \sum_{M \in \mathcal{M}} P(M)P(w|M)\prod_{i=1}^kP(q_i|M)
\end{equation*}
\normalsize
where $\mathcal{M}$ is the set of feedback document models. $\mathcal{M}$ consists of top-1000 documents retrieved by searching for query+aspect.\\

{\bf 4) Search result diversification using xQUAD.} In addition to adding aspect explicitly to the query, we considered a state of the art diversification baseline. xQUAD  \cite{Santos:2010:EQR:1772690.1772780} is a ranking framework that uses sub-queries to diversify the results so that all aspects of an under-specified query are addressed in the results. We use $TKB$ to formulate sub-queries for the given query and aspect. For example, for a query \term{<autoencoder application>}, the sub-queries that we use were \term{<autoencoder application e>} where $e$ is an entity connected to \term{autoencoder} via \term{application} relation in $TKB$. \\
{\bf 5) Neural Networks for classification (HANN).} We used hierarchical attention neural networks \cite{Yang2016HierarchicalAN} {\bf (HANN)} for classifying the paper/abstract into one/more/none of the 3 categories: \term{algorithm}, \term{application} and \term{implementation}. The training data consisted of 1500 annotated documents. These were collected by following the scheme as described in Section \ref{sec:eval_scheme}. The training was done for 200 epochs after which the accuracy started converging. Top 1000 candidate documents retrieved according to query likelihood model (used in Equation \eqref{eq:query_likelihood}) for each query were re-ranked according to the following equation:
\begin{equation*}
    P(d|q,a) = HANN(d,a)*P(d|q)
\end{equation*}

where $HANN(d,a)$ is the probability of the document being classified into aspect $a$ returned by the neural network classifier. $P(d|q)$ is estimated using Equation \eqref{eq:query_likelihood}.\\
\end{comment}

%Above baselines are compared against our Mixture Model (MM) given in Eq. \eqref{eq:kl_divergence}. 
%\noindent{\bf 4) Mixture Model (MM).} This is our retrieval model indicated by {\bf MM} and described by Eq. \eqref{eq:model_eq}. Top 1000 documents retrieved according to query-likelihood model were re-ranked.The documents were returned in increasing order of KL-divergence as described in Eq. \eqref{eq:kl_divergence}.
%\vspace*{-4mm}
\subsection{Evaluation scheme and metrics}
%\vspace*{-5mm}
{\bf Evaluation scheme.} 
\label{sec:eval_scheme}
In the absence of an extensive ground-truth dataset, we conducted a crowd-sourced user-evaluation exercise (involving Computer Science students and researchers, not related to the project) to measure the performance of our model. %We built a web-based interface to facilitate the evaluations. We recruited students and researchers of Computer Science (not directly related to the project) to conduct the evaluations. They were asked to evaluate the top-5 documents returned by our method as well as competing techniques for pairs of a given query and an aspect. Because determining if a paper addresses a particular aspect is a subjective question, we formulated domain specific rules with the help of in-house experts to determine the relationship between the query and the retrieved paper. 
We formulated domain-specific questions, and depending on the answers marked by the evaluators, the documents were assigned a particular score for a query and aspect pair.
\begin{comment}
Below we briefly describe how the papers are assigned scores and categorised into each aspect for a query:\\
\begin{compactenum}
\item {\bf Application.} If the query entity is used as a solution in the problem identified by the paper, then the paper addresses application aspect for the query and score of 1 is assigned. In other cases, a score of 0 is assigned. For example, in the paper ``Exploring autoencoders for unsupervised feature selection'', \term{autoencoder} is used for feature selection, so this paper qualifies for application aspect for \term{autoencoder} whereas ``Parallelizing the Sparse Autoencoder" does not.
\item {\bf Algorithm.} If the query forms the problem and an algorithm is proposed or improved as a solution, then a score of 3 is assigned. If the query forms the solution and an algorithm is proposed in the paper, then a score of 2 is assigned. If an algorithm is used but not proposed in the paper, then a score of 1 is assigned. In other cases, 0 is assigned. For example, the paper ``An adaptive constant time hashing scheme for dynamic key set" gets a score of 3 for \term{hashing} while ``Sampling Based N-Hash Algorithm for Searching Frequent Itemset" gets a score of 2.
\item {\bf Implementation.} If the query forms the problem and a solution is proposed that deals with one of the following -- 1) improving the run-time/space complexity or 2) building a software/prototype implementation, then a score of 2 is assigned. If the query forms the solution which deals with one of the above mentioned cases, then a score of 1 is assigned. In other cases, 0 is assigned. For example, ``Genetic Ant Algorithm for Continuous Function Optimization and Its MATLAB Implementation" gets a score of 2 for \term{genetic\_algorithm} while ``A Novel Approach towards FPGA Implementation of a Multiple Parameter Optimization Technique using Genetic Algorithm" is scored 1.
\end{compactenum}
\end{comment}
\\
\noindent{\bf Evaluation metrics.}
Each query and abstract pair was graded by at least 2 evaluators. We converted the response from each of them into a graded relevance scale and averaged the relevance values marked by them for each query-abstract pair. We used {\bf Discounted Cumulative Gain (DCG)} and {\bf Precision} to evaluate top-5 documents.
%\vspace*{-4mm}
\subsection{Results and Discussions}
%\vspace*{-3mm}
Table \ref{tab:algorithm_results} shows the results for \aspect{algorithm}, \aspect{application} and \aspect{implementation} aspects. We observe that our model outperforms the rest of the baselines in terms of precision@5 and DCG for all of the 3 aspects. {\bf QL + query + aspect + QE} comes second after our retrieval model. By modelling the aspect and query dependant probability explicitly, we were able to address the problems of simple keyword-based match for aspects described in Section \ref{sec:intro} and \ref{sec:model}. For example, the top-2 papers retrieved for \term{genetic\_algorithm} for application aspect by our model were \emph{Genetic Ant Algorithm for Continuous Function Optimization and Its MATLAB Implementation} and \emph{Solve Zero-One Knapsack Problem by Greedy Genetic Algorithm}. The top-2 papers retrieved by {\bf QL + query + aspect + QE} for \aspect{application} aspect do not describe any application of \term{genetic\_algorithm} but contained a few terms like ``a wide application prospect" in the abstract due to which it was retrieved in the top positions. Adding relevance feedback terms also did not work because the list of pseudo relevant documents did not contain relevant documents in the first place due to plain keyword-based retrieval. Both the papers retrieved by our method address application aspect for \term{genetic\_algorithm} even if ``application" is not mentioned in the title. 
\vspace{-4mm}
\begin{table*}[t]
\caption{Results for algorithm, application and implementation aspect.}
\label{tab:algorithm_results}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{p{3cm}p{1.25cm}p{0.75cm}p{0.75cm}p{1.25cm}p{0.75cm}p{0.75cm}p{1.25cm}p{0.75cm}p{0.75cm}}
\toprule
%{\bf & & & & & & \\ \hline}
& \multicolumn{3}{c}{\textbf{Algorithm}} & \multicolumn{3}{c}{\textbf{Application}} & \multicolumn{3}{c}{\textbf{Implementation}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
{\bf Approach} &  {DCG@5} &  {P@5}  & {P@1} &  {DCG@5} &  {P@5}  & {P@1} &  {DCG@5} &  {P@5} & {P@1}  \\ \midrule
{\bf MM} & {\bf 6.27} & {\bf 0.70} & {\bf 0.75}  & {\bf 2.64} & {\bf 0.45} & {\bf 0.47} & {\bf 2.33} & {\bf 0.44} & 0.40 \\ 
{\bf QL+query} & 2.69 & 0.3 & 0.33 & 1.42 & 0.25 & 0.22 & 1.05 & 0.16 & 0.23 \\ 
{\bf QL+query+aspect} & 5.03 & 0.56 & 0.59 & 2.38 & 0.41 & 0.35 & 1.92 & 0.30 & \em{0.43} \\ 
{\bf QL+query+aspect+QE} & \em{5.12} & \em{0.58} & \em{0.61} &  \em{2.5} & \em{0.43} & \em{0.41} & \em{2.29} & \em{0.37} & {\bf 0.49} \\ \bottomrule
\end{tabular}}

%\vspace{-5mm}
\end{table*}
\normalsize

\begin{comment}
\begin{table*}
\caption{Top-2 papers retrieved for \term{genetic\_algorithm} along \aspect{application} aspect}
\label{tab:application_examples}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{20mm}@{\hspace{1em}}p{48mm}@{\hspace{1em}}p{40mm}}\\
\toprule
{\bf Approach} & Paper retrieved at k=1 & Paper retrieved at k=2 & \\
\midrule
\multirow{1}{*}{\textbf{MM}} & Genetic Ant Algorithm for Continuous Function Optimization and Its MATLAB Implementation &   Solve Zero-One Knapsack Problem by Greedy Genetic Algorithm \\ \hline
\multirow{1}{*}{\parbox{2cm}{\textbf{QL + query + aspect + QE}}} & Recent Developments in Evolutionary and Genetic Algorithms: Theory and Applications & Comparison and Analysis of Different Mutation Strategies to improve the Performance of Genetic Algorithm  \\ \bottomrule
\end{tabular}
}
\label{tab:top-2_examples}

\end{table*}
\end{comment}

 %Our KB consists of paths between \term{reinforcement\_learning} and \term{fuzzy\_control\_system} through \term{artificial\_intelligence} as follows: \\
%\triple{fuzzy\_control\_system, technique, process\_control},\\ \triple{process\_control, application, control\_theory},\\  \triple{control\_theory, research, artificial\_intelligence} and \\ \triple{reinforcement\_learning, technique, genetic\_algorithm},\\ \triple{genetic\_algorithm, approaches, machine\_learning},\\ \triple{machine\_learning, technique, artificial\_intelligence}. So, the documents that contain terms from \term{fuzzy\_control\_system} were ranked higher even if ``application" was not explicitly mentioned. Similarly, there is a length 5 meta-path between \term{ontology} and \term{similarity\_search} as follows:
%\triple{ontology, data\_structurefor, conceptual\_schema}, \triple{conceptual\_schema, data\_structurefor\_inverse, conceptual\_graph}, \triple{conceptual\_graph, typeof, graph}, \triple{graph, explores\_inverse, search\_algorithm}, \triple{search\_algorithm, typeof\_inverse, similarity\_search}. Therefore, this document was ranked highest by our method. 


\begin{comment}

{\bf Implementation aspect}
Our model beat other baselines for implementation aspect. It obtained a precision of 0.53 and DCG value of 3.20. {\bf QL+ query+ aspect+ QE} came next with a precision of 0.52 and DCG 2.96. {\bf QL+query+aspect} obtained a precision of 0.46 and DCG 2.65. The neural network model performed poorly for this aspect as well with a precision of 0.28 and DCG 1.72.
Table \ref{tab:top-5_implementation} lists top-5 papers retrieved for the query \term{autoencoder} by our model as well as baselines {\bf Ql+query+aspect} and {\bf QL+query+aspect+QE}. We can see here that the presence of the word ``implement" in the document does not necessarily imply that the paper addresses the implementation aspect. For example, the paper titled \emph{Mirrored STDP Implements Autoencoder Learning in a Network of Spiking Neurons} is not a paper that addresses implementation aspect for autoencoder.  Our model retrieved the paper titled \emph{Parallelizing the Sparse Autoencoder} at the top position. This happened because it contained terms like ``parallelize", which is a very strong indicator of implementation aspect independent of the query. The paper titled \emph{Memristor crossbar based unsupervised training using autoencoders \& Autoencoder using kernel method} was retrieved at the 2nd position. It was due to the presence of words like ``memristor", ``computation", ``power" or ``chip" (in the abstract and title) which have a high probability of being seen if the aspect is implementation as well as the presence of query-dependent terms like ``feature" and ``extraction" for \term{autoencoder}. (there are two triples -- \triple{feature\_selection, application, artificial\_neural\_network} and \triple{artificial\_neural\_network, type\_inverse, autoencoder}). However, only a few of these terms appear in the list of 100 feedback terms generated by {\bf QL + query + aspect + QE}. Apart from that, documents containing query dependent terms like were also ranked higher in our model because we generate the final probability distribution by mixing the query-independent as well as query-dependent component. 
\end{comment}



==> Aspect-based Academic Search using Domain-specific KB/introduction.tex <==
%\vspace*{-5mm}
\section{Introduction}
%\vspace*{-3mm}
\label{sec:intro}
Academic search engines such as Google Scholar,
%,\footnote{\url{https://scholar.google.com}} 
PubMed,
%\footnote{\url{https://ncbi.nlm.nih.gov/pubmed/}} 
and Semantic Scholar
%,\footnote{\url{https://semanticscholar.org}} 
play a central role in the lives of researchers dealing with the ever growing flood of related work. To further improve the academic search experience, there have been proposals to either re-rank the results using user's interests~\cite{Sugiyama:2015:CES:2785536.2785566} and the set of papers assessed relevant~\cite{doi:10.1108/EL-04-2017-0077}, or to recommend new articles based on a query article~\cite{Chakraborty:2016:FFR:2990640.2990686}.

In this paper, we define and solve a novel academic search task, called \emph{aspect-based retrieval}, which is targeted towards enabling the academic search user to specify the \emph{aspect} along with the query to retrieve a ranked list of scientific articles that are (i) relevant to the query, and (ii) the relevance relation \cite{bean2001} between the query and retrieved documents is semantically close to the specified aspect. We illustrate this expected behavior with a concrete example: consider the query \term{\footnotesize{autoencoder}} and an aspect of interest, say, \aspect{\footnotesize{application}}, then we aim to rank high the articles which are related to the concept of \term{\footnotesize{autoencoder}} \emph{and} are about the \textit{applications} of autoencoders. If there were two papers, titled (a) ``Complex-valued Autoencoders'' and (b) ``Exploring autoencoders for unsupervised feature selection'', our system should rank the paper (b) higher than paper (a) since it specifically deals with applications of the specified query rather than its variants. Note that both papers are indeed relevant to the central concept being queried. Aspect-based retrieval of scientific documents is not straightforward at all since the relation semantics do not manifest as simple keyword matches. Simply expanding the query with terms that define the aspect fails to retrieve relevant articles. In the above example, the paper (b) does not contain the \term{\footnotesize{application}} in the title as well as the abstract. On the other hand, a document, titled ``Evaluating the Performance of Dynamic Database Applications'' is not related to the query \term{\footnotesize{ RDBMS}} along the \aspect{\footnotesize{application}} aspect although its title contains the term \term{\footnotesize{applications}}. The way in which the specified semantic relationship manifests between the query and a document is highly dependent on the domain we operate in.
For example, given the query \term{\footnotesize{autoencoder}}, for a document to be related along \aspect{\footnotesize{application}} aspect, the presence of terms like \term{\footnotesize{feature}} or \term{\footnotesize{selection}} with terms similar to \term{\footnotesize{application}} would be highly suggestive because \term{\footnotesize{feature\_selection}} is known to be an application of \term{autoencoder}. But this can not be easily determined by just analysing the documents without prior knowledge of the domain.
%%%%%%%%%%%%%%%%%%%%

%%%%%%-----------------As we show later, this is not just an idiosyncratic example. The problem appears in many other cases. It should be noted that although our work closely resembles the faceted retrieval~\cite{Gupta:2018:GSA:3197026.3203900,Wu:2011:IAW:2016945.2016963}, unlike faceted retrieval systems it does not generate and evaluate of quality of facets given a query. Instead we focus on ranking relevant documents given a query and a facet. In academic search, techniques have been proposed to retrieve relevant papers along their citation context in a query document~\cite{Chakraborty:2016:FFR:2990640.2990686}.

 



%\subsection{Our Approach}
We address the challenge of aspect-oriented retrieval for scientific documents by minimizing the risk of returning a document whose language model diverges from the model estimated for domain-specific query and aspect specified by the user. The query and aspect models are derived using domain-specific knowledge bases (KBs), which is challenging in itself due to the inherent sparsity of relations in these KBs. By using a domain-specific KB of computer science, like TeKnowbase \cite{Upadhyay:2018:CAT:3184558.3191532}, we show how to overcome the sparsity issue in KB via inference using meta-paths derived from the KB. Our results over the Open Research Corpus~\cite{ammar:18} dataset containing more than 39 million published research papers show that our proposed approach outperforms variants of query likelihood language models with/without relevance feedback. 
%Some example relevant papers retrieved at top-5 positions by our proposed model for 2 queries along different aspects is shown in Table~\ref{tab:examples}.%\todo{some discussion on metapath should come here}

%In this paper, we have addressed the problem of aspect-based retrieval for scientific literature. We have developed a retrieval model that returns a ranked list of articles given a query and an aspect. The primary idea is to estimate a language model for the aspect as well as the query and use a mixture of the two to determine the relevance of the article. We need extensive domain knowledge to estimate the language model for the query and the aspect. To do this, we have used the relationships in a technical knowledge base to represent aspects. We have further used meta-paths in the knowledge base to infer relationships between entities to address sparsity of knowledge base links. To the best of our knowledge, our work is the first of its kind in academic search.
\begin{comment}
\begin{table*}[t]
\caption{Titles of Example Relevant Papers for Queries along Specified Aspects}
\label{tab:examples}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{20mm}@{\hspace{1em}}p{40mm}@{\hspace{1em}}p{40mm}@{\hspace{1em}}p{40mm}}
\toprule
{\bf Query} &  \aspect{Application} & \aspect{Algorithm} & \aspect{Implementation} \\
\midrule
\term{cryptography} & Cryptographic Protection of Computer-Based Data Files &  Cryptographic algorithm on multicore processor: A review & Design of a Reconfigurable Hardware for Efficient Implementation of Secret Key and Public Key Cryptography \\ \cmidrule{1-4}
\term{autoencoder} & Exploring autoencoders for unsupervised feature selection & Training Stacked Denoising Autoencoders for Representation Learning & Parallelizing the Sparse Autoencoder \\ %\cmidrule{1-4}
%\term{neural\_ network} & Application of Particle Swarm Optimization and RBF Neural Network in Fault Diagnosis of Analogue Circuits & Evolutionary Neural Network Based on New Ant Colony Algorithm & Design of FPGA based general purpose neural network \\\cmidrule{1-4}
%\term{hashing} & Sampling Based N-Hash Algorithm for Searching Frequent Itemset & An Alternative Analysis of the Open Hashing Algorithm & Low Power And Area Efficiency of SHA-1 \\
\bottomrule
\end{tabular}
}
\end{table*}
\end{comment}
\begin{comment}
\noindent {\bf Contributions.} We summarize our main contributions below: 
\begin{compactenum}
\item introduce the novel task of query aspect-based retrieval for scientific literature,%\todo{is this our contribution? it has been done before}
\item develop a new retrieval model by making use of a domain-specific knowledge base, and
\item propose an algorithm to overcome the sparsity issues in domain-specific KBs by using metapaths to infer relationships and improve the query-aspect language model.
\end{compactenum}
We experimentally evaluate our proposal using a large corpus of published research papers and show performance improvements over a variety of baselines.
\end{comment}
\sbjcomment{Our aim is to build a system that retrieves papers given a query and an aspect. The main contributions of this paper are as follows:\\
{\bf 1)} Introduced the problem of query dependent aspect-based retrieval for scientific literature.\\
{\bf 2)} Proposed a retrieval model to retrieve relevant papers addressing a given aspect for a query using a technical knowledge base.\\
{\bf 3)} Proposed an algorithm that uses meta-paths in a technical knowledge base to infer relationships between its entities.\\}
%\vspace{-7pt}
%\todo{section arrangement is not needed in a conf paper. u can add sec no with the contribution}

==> Aspect-based Academic Search using Domain-specific KB/model.tex <==
%\vspace*{-2mm}
\section{Aspect based retrieval model}
%\vspace*{-2mm}
\label{sec:model}
\begin{comment}
\begin{figure}[!h]
\centering
\subfloat[] {\includegraphics[width=0.2\textwidth]{figs/q_ind.pdf}} \hfill
\subfloat[] {\includegraphics[width=0.3\textwidth]{figs/q_dep.pdf}}\hfill
\subfloat[] {\includegraphics[width=0.35\textwidth]{figs/scoring.pdf}}\hfill
\caption{Components of the mixture distribution. a) The query independent component defines a probability distribution $P(w|a)$ on terms based on the aspect alone. For \aspect{application} aspect, terms like \term{application} or \term{usage} are assigned high probabilities. b) The query and aspect dependent component uses relationships in a domain specific knowledge graph to assign probabilities $P(w|q,a)$ to terms. For a query \term{autoencoder} and \aspect{application} aspect, terms present in entities connected by the \term{application} relation to \term{autoencoder} are assigned high probabilities. c) The final distribution is determined by a mixture of estimated $P(w|a)$ and $P(w|q,a)$.  The documents are ranked in decreasing order of divergence of their language models with that of the estimated mixture model}
\label{fig:system}
\end{figure}
\end{comment}
\subsection{System overview}
%\vspace*{-1mm}
Our system takes a query and an aspect as input, and returns a ranked list of relevant documents. Users express their information need as strings of words called {\bf queries}. In our case, a query is a technical entity. An {\bf aspect} is the relevance relation specified by the user between the query and the relevant document. 
%%%%%%%%%%%
%For example, for the query \term{autoencoder}, a paper titled \emph{Exploring autoencoders for unsupervised feature selection} is more relevant for the \emph{application} aspect.
%%%%%%%
Given a query, the documents are ranked using retrieval models \cite{Manning:2008:IIR:1394399}. A {\bf retrieval model} transforms the document space into an intermediate representation and returns a ranked list of documents according to some scoring function. %Our idea is to estimate a language model \cite{Ponte:1998:LMA:290941.291008} for each aspect and use it as a prior to score the documents.

%Our system takes a query and an aspect as input and returns a ranked list of relevant documents. We use a generative framework to model documents addressing an aspect for a query. Given an aspect, the document is generated according to a probability distribution described by the aspect alone, which is the prior. The query and aspect together model the document according to some other distribution. The final distribution is a mixture of the two. We describe the model and the estimation techniques more formally in the following paragraphs.
%\vspace*{-2mm}
\subsection{Retrieval model and Estimation}
%\vspace*{-2mm}
Language modelling techniques \cite{Ponte:1998:LMA:290941.291008} model the relevance of a document as the probability of generating the query from the document. Expanding the query with aspect terms and doing relevance feedback \cite{Lavrenko:2001:RBL:383952.383972}  will only retrieve documents containing those terms. Given a query $q$ and an aspect $a$, a relevant document $d$ consists of terms determined by both $q$ and $a$. 

\noindent {\bf Aspect dependent prior probability.}
\label{sec:term_prior}
$P(w|a)$ is the prior, which is the probability of a term $w$ appearing in $d$ given an aspect $a$, independent of the query. 

\noindent {\bf Query and aspect dependent probability.}
The probability of a term appearing in $d$ given a query $q$ and aspect $a$ is denoted by $P(w|q,a)$.

\noindent {\bf Mixture of the two probability distributions.}
The relevance of $d$ will be determined by a mixture model of both the probability distributions. Equation \eqref{eq:model_eq} describes our probability distribution. It is denoted as $MM$.
%\vspace*{-2mm}
\small
\begin{equation}
%\vspace*{-2mm}
\label{eq:model_eq}
    MM(w) = \lambda P(w|a) + (1-\lambda)P(w|q,a)
\end{equation}\label{eq2}
\normalsize
\noindent
\noindent {\bf Scoring of documents.}
The language model $M_d$ of a candidate document is expressed by Eq. \eqref{eq3}. Dirichlet smoothing is used for $M_d$.
%\vspace*{-2mm}

\small
 \begin{equation}
 \label{eq3}
M_d(w) = \frac{tf(w,d) + \mu P(w|C)}{length(d)+\mu}
 \end{equation}
 \normalsize
 where $tf(w,d)$ is the frequency of $w$ in $d$, and $P(w|C)$ is the probability of $w$ appearing in the entire collection. The risk associated with using $MM$ to approximate $M_d$ is expressed by KL-divergence between $MM$ and $M_d$ and the documents are returned in an order of increasing KL-divergence.
%\vspace*{-2mm}
\small
\begin{equation}
%\vspace*{-2mm}
\label{eq:kl_divergence}
    KL(MM||M_d) = \sum_{w} P(w|MM)\log\frac{P(w|MM)}{P(w|M_d)}
\end{equation}
\normalsize

%\subsection{Estimation}
%\label{sec:estimation}
%We indexed the Open Research Corpus dataset on Galago to estimate aspect-dependent probability. We later conduct our experiments on the same dataset (described in Section \ref{sec:experiment}).
%The dataset we use....

\noindent{\bf Estimation of query-independent component.}
\label{sec:query_independent}
$P(w|a)$ is estimated using a narrow set of documents from our dataset acquired as follows. We chose 10 queries and retrieved the top 10 documents for them using the standard query likelihood model. Additionally, we fired queries of the form ``query+aspect" to retrieve the top-10 documents using the same model.  We recruited evaluators to annotate about 1500 documents with the aspect labels (described in details in Section \ref{sec:eval_scheme}). In order to increase the size of our document set, we used heuristics to collect more documents given an aspect. We formulated a query containing only the aspect as a keyword and retrieved documents for it using the standard likelihood model. But, we retained only those documents which contained the name of the aspect in the title on the intuition that such documents are highly likely (though not guaranteed) to be about those aspects. Having a set of ground-truth documents $D$, $P(w|a)$ is estimated according to Equation \eqref{eq:term_prior}.
\small
\begin{equation}
%\vspace*{-2mm}
\label{eq:term_prior}
    P(w|a) = \frac{1}{|D|} \sum_{d \in D} \frac{tf(w,d)}{\sum_{w' \in d}tf(w',d)}
\end{equation}
%\vspace*{-2mm}
\normalsize
%\vspace*{-1mm}
\noindent{\bf Estimation of query-dependent component.}
We used relationships in TeKnowbase ($TKB$)  \cite{Upadhyay:2018:CAT:3184558.3191532} to represent aspects. $TKB$ consists of entities such as \term{\footnotesize{hidden\_markov\_model}} or \term{\footnotesize{ speech\_r\-ecognition}} and other domain-specific relationships like \term{\footnotesize{application}}, \term{implemen\-tation} or \term{algorithm}. 
The triple \triple{speech\_\-recognition, application, hidden\_mar\-kov\_model} conveys information that \term{speech\_recognition} is an application of \term{hidden\_m\-arkov\_model}. The entities connected via \term{application} relation in $TKB$ have a higher probability of appearing in documents addressing \aspect{application} aspect. However, $TKB$ is sparse. To automatically infer the entities participating in a particular relationship type, we used meta-paths. A meta-path is a sequence of edges with labels connecting two nodes which have been used previously for KB completion tasks \cite{Lao:2011:RWI:2145432.2145494}, link prediction \cite{journals/pvldb/Ley09} as well as to find similarity between two nodes \cite{5992571,Shi:2012:RSH:2247596.2247618}. Figure \ref{fig:meta_path_application} shows how meta-paths can be used to infer relationships between entities. 
%\vspace*{-1mm}
\begin{figure}[!h]
\vspace*{-3mm}
\centering
\subfloat[] {\includegraphics[width=0.5\textwidth]{figs/meta-path_application_a.pdf}} \hfill
%\subfloat[] {\includegraphics[height=0.9in]{figs/hmm.pdf}} \hfill
\subfloat[] {\includegraphics[width=0.5\textwidth]{figs/meta-path_application_b.pdf}}\hfill
%\subfloat[] {\includegraphics[height=0.9in]{figs/autoencoder_infer.pdf}}\hfill
\caption{Examples of meta-paths for \term{application} relation. (a) The meta-path \triple{application, type\_inverse} exists between \term{speech\_recognition} and \term{hidden\_markov\_model}. (b) \term{feature\_selection} and \term{autoencoder} are not related by \term{application} relation but still it can be inferred because of the existence of the same meta-path \triple{application, type\_inverse} between them.}
\label{fig:meta_path_application}
\vspace*{-4mm}
\end{figure}
%\vspace*{-1mm}

\noindent {\bf 1) Direct inference using meta-paths.}
To automatically determine entities that participate in a given relationship type with entity $e_i$, we used the path-constrained random walk algorithm ($PRA$) proposed in \cite{Lao:2011:RWI:2145432.2145494}. Given a set $E$ of entities in $TKB$, a source node $e_i$ and a meta-path $P$, a path-constrained random walk defines a probability distribution $h_{e_i,P}(e_j)$ to all entities in $E$ which is the probability of reaching $e_j$ from $e_i$ by doing a random walk along $P$. The key idea is to acquire the set of meta-paths representing the given relationship type and use $PRA$ for inferencing. To do so, we retrieved the set of all meta-paths ($MP$) connecting the given relationship type in $TKB$ and scored them according to their frequency. Given a set of meta-paths $MP = P_1, P_2,..., P_n$, the score for each node reachable from source $e_i$ is given by:
$\label{eq:path_constrained}
  score_{e_i}(e_j) =  \alpha_1h_{e_i,P_1}(e_j) + \alpha_2h_{e_i,P_2}(e_j) + ... + \alpha_nh_{e_i,P_n}(e_j),
$
where $\alpha_l (l=1 \ldots n)$ is the frequency of meta-path $P_l$. $score_{e_i}(e_j)$ is converted to a probability distribution using \emph{softmax} and denoted by Equation \eqref{eq:softmax_direct}. \\%Since we have to estimate a probability distribution, we converted $score_{e_i}(e_j)$ to a probability distribution using softmax and denote it as $DI_{e_i}(e_j)$.
%\vspace*{-2mm}



\noindent {\bf 2) Indirect inference using meta-paths.}
\label{sec:metapath2vec}
$PRA$ assigns zero probability to nodes that are not reachable via any meta-paths in $MP$. To address this issue, we used MetaPath2Vec \cite{Dong:2017:MSR:3097983.3098036}. It takes a meta-path as input and constructs embeddings of entities such that entities that are likely to be connected via the meta-path (and not necessarily having a meta-path between them) are assigned vector representations closer to each other.  We used the top-k meta-paths in $MP$ as input to metapath2vec and obtained vector representations $V_e$ for entity $e$. We used the softmax function to convert cosine similarities between entities into a probability distribution as described in Equation \eqref{eq:softmax_indirect}.

\noindent\begin{minipage}{5.7cm}
\small
\begin{equation}
%\vspace*{-2mm}
\label{eq:softmax_direct}
    DI_{e_i}(e_j) = \frac{e^{score_{e_i}(e_j)}}{\sum_{e_{k} \in |E|} e^{score_{e_i}(e_{k})}}
\end{equation}
\end{minipage}
\begin{minipage}{6.5cm}
\small
\begin{equation}
\label{eq:softmax_indirect}
h'_{e_i}(e_j) = \frac{e^{\mathrm{sim}\left(V\left(e_i\right), V\left(e_j\right)\right)}}{\sum_{e_{k} \in |E|} e^{\mathrm{sim}\left(V\left(e_i\right), V\left(e_k\right)\right)}}.
\end{equation}
\end{minipage}
\normalsize

The probability distribution for inferencing is a mixture of $DI_{e_i}(e_j)$ and $h'_{e_i}(e_j)$ using $\beta$ as given in Eq. \eqref{eq:mix_ent_prob}. Since the documents are represented as bag of words, we defined the distribution over terms instead of entities using Eq. \eqref{eq:query_aspect_prob}. $terms(e)$ is the set of words present in the entity $e$, and $e_q$ is the entity that $q$ represents. The final probability is a mixture given by Equation \eqref{eq:model_eq}.
%\vspace{-2mm}
\small
\begin{equation}
\vspace*{-2mm}
\label{eq:mix_ent_prob}
    P_{a}(e_i|e_j) = \beta*DI_{e_i}(e_j) + (1 - \beta)*h'_{e_i}(e_j)
\end{equation}
%\vspace{-2mm}
\begin{equation}
\vspace*{-2mm}
\label{eq:query_aspect_prob}
    P(w|q,a) = \sum_{e}P_{a}(e|e_q), \text{s.t. $w \in terms(e)$}
\end{equation}
%\vspace{-2mm}

\normalsize
%Equation \eqref{eq:term_prior} estimates the prior probability of the term given only the aspect. Equation \eqref{eq:query_aspect_prob} estimates the probability of a term given the query and the aspect both. 

%of $P(w|a)$ and $P(w|q,a)$. $\lambda$ is used to mix the two distributions. The final distribution, as described at the beginning of the section is given below:

==> Aspect-based Academic Search using Domain-specific KB/related_work.tex <==
\section{Related Work}
\label{sec:related}

\noindent{\bf Aspect-based search or faceted search:} Aspect-based or faceted search allows users to retrieve documents along different dimensions. In the context of regular search, \cite{HearstFacettedBrowsing} proposed design interfaces for hierarchical faceted search. \cite{Tunkelang2006DynamicCS}  addressed the vocabulary problem for faceted search. \cite{Koren:2008:PIF:1367497.1367562} developed a personalized faceted retrieval system. In all of these systems, the facets are predefined properties directly mapped to the document. In our case, we do not know the mapping between the facet value and the document. The retrieval model that we propose returns a ranked list of documents given a query and facet/aspect as input.

\noindent{\bf Aspect generation and identification:} In many cases, the standard facets/aspects are not enough to provide a great user experience \cite{Wu:2011:IAW:2016945.2016963}. In such scenarios, they have to be automatically generated. \cite{Wu:2011:IAW:2016945.2016963,Gupta:2018:GSA:3197026.3203900,7728095}  proposed methods to \emph{generate} aspects for queries and evaluates these aspects based on correctness and novelty. This is different from our work because we are interested in retrieving relevant documents given a query and an aspect. We can use these techniques to generate aspects for our setting and then use our model to retrieve documents relevant to the generated aspects.

 In the context of academic search, research paper recommendation has been thoroughly studied and a number of systems have been developed for the same. These include recommendation tools that retrieve papers based on the user's interest \cite{Sugiyama:2015:CES:2785536.2785566,DBLP:journals/corr/abs-1304-5457} or similar to a given set of papers \cite{doi:10.1108/EL-04-2017-0077}. \cite{gipp2009scienstein} built \emph{Scienstein} that allows users to search for papers using authors or reference lists apart from the usual keyword-query search. These tools make use of the underlying structure of the citation graph as well as machine learning techniques on the document text. \cite{Diederich:2007:DSG:1255175.1255305} made an effort to provide faceted retrieval for research papers in computer science. The facets were -- publication years, authors or conferences. These facets are different from aspects in our scenario. \cite{Chakraborty:2016:FFR:2990640.2990686}  proposed techniques to further categorise the relationships between the query paper and the recommended paper. These relationships are expressed in the form of facets like \term{background}, \term{alternative\_approaches}, \term{methods} and \term{comparisons}.  \cite{Cohan2018} used similar facets to summarize scientific papers. These facets are extracted by identifying the context of the text surrounding the citation.  Although these facets are similar to aspects in our problem, they describe the relationship between two papers unlike our case where the relationship has to be identified between a keyword query and the paper. 

To the best of our knowledge, aspect-based retrieval for scientific articles is a novel problem. The aspects that we define in our paper have not been explored for academic search till now. Using relationships in a domain-specific knowledge graph to represent these aspects, our system infers these relationships using meta-paths between its entities to address sparsity issues.   %\todo{add other points how u overcome existing limitations}

==> related_work.tex <==
\section{Related Work}
\label{sec:related}

\noindent{\bf Aspect-based search or faceted search:} Aspect-based or faceted search allows users to retrieve documents along different dimensions. In the context of regular search, \cite{HearstFacettedBrowsing} proposed design interfaces for hierarchical faceted search. \cite{Tunkelang2006DynamicCS}  addressed the vocabulary problem for faceted search. \cite{Koren:2008:PIF:1367497.1367562} developed a personalized faceted retrieval system. In all of these systems, the facets are predefined properties directly mapped to the document. In our case, we do not know the mapping between the facet value and the document. The retrieval model that we propose returns a ranked list of documents given a query and facet/aspect as input.

\noindent{\bf Aspect generation and identification:} In many cases, the standard facets/aspects are not enough to provide a great user experience \cite{Wu:2011:IAW:2016945.2016963}. In such scenarios, they have to be automatically generated. \cite{Wu:2011:IAW:2016945.2016963,Gupta:2018:GSA:3197026.3203900,7728095}  proposed methods to \emph{generate} aspects for queries and evaluates these aspects based on correctness and novelty. This is different from our work because we are interested in retrieving relevant documents given a query and an aspect. We can use these techniques to generate aspects for our setting and then use our model to retrieve documents relevant to the generated aspects.

 In the context of academic search, research paper recommendation has been thoroughly studied and a number of systems have been developed for the same. These include recommendation tools that retrieve papers based on the user's interest \cite{Sugiyama:2015:CES:2785536.2785566,DBLP:journals/corr/abs-1304-5457} or similar to a given set of papers \cite{doi:10.1108/EL-04-2017-0077}. \cite{gipp2009scienstein} built \emph{Scienstein} that allows users to search for papers using authors or reference lists apart from the usual keyword-query search. These tools make use of the underlying structure of the citation graph as well as machine learning techniques on the document text. \cite{Diederich:2007:DSG:1255175.1255305} made an effort to provide faceted retrieval for research papers in computer science. The facets were -- publication years, authors or conferences. These facets are different from aspects in our scenario. \cite{Chakraborty:2016:FFR:2990640.2990686}  proposed techniques to further categorise the relationships between the query paper and the recommended paper. These relationships are expressed in the form of facets like \term{background}, \term{alternative\_approaches}, \term{methods} and \term{comparisons}.  \cite{Cohan2018} used similar facets to summarize scientific papers. These facets are extracted by identifying the context of the text surrounding the citation.  Although these facets are similar to aspects in our problem, they describe the relationship between two papers unlike our case where the relationship has to be identified between a keyword query and the paper. 

To the best of our knowledge, aspect-based retrieval for scientific articles is a novel problem. The aspects that we define in our paper have not been explored for academic search till now. Using relationships in a domain-specific knowledge graph to represent these aspects, our system infers these relationships using meta-paths between its entities to address sparsity issues.   %\todo{add other points how u overcome existing limitations}
